CORE: a Complex Event Recognition Engine

Complex Event Recognition (CER) systems are a prominent technology for finding user-defined query patterns over large data streams in real time. CER query evaluation is known to be computationally challenging, since it requires maintaining a set of partial matches, and this set quickly grows super-linearly in the number of processed events. We present CORE, a novel COmplex event Recognition Engine that focuses on the efficient evaluation of a large class of complex event queries, including time windows as well as the partition-by event correlation operator. This engine uses a novel automaton-based evaluation algorithm that circumvents the super-linear partial match problem: under data complexity, it takes constant time per input event to maintain a data structure that compactly represents the set of partial matches and, once a match is found, the query results may be enumerated from the data structure with output-linear delay. We experimentally compare CORE against state-of-the-art CER systems on real-world data. We show that (1) CORE's performance is stable with respect to both query and time window size, and (2) CORE outperforms the other systems by up to five orders of magnitude on different workloads.

==> extras/keywords.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>10010520.10010553.10010562</concept_id>
%   <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010575.10010755</concept_id>
%   <concept_desc>Computer systems organization~Redundancy</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10010520.10010553.10010554</concept_id>
%   <concept_desc>Computer systems organization~Robotics</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>10003033.10003083.10003095</concept_id>
%   <concept_desc>Networks~Network reliability</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{complex event recognition, automata, enumeration}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main/main"
%%% End:


==> sections/competitors.tex <==
\subsection{Competitors}

(Internal note: for a description of the capabilities/papers/context of the systems below, see the more detailed comparison at \url{https://github.com/DomagojVrgoc/CEP/blob/master/systems/summary.md})

We consider the following competitor systems.

\begin{itemize}
\item SASE
\item Esper
\item Tesla/T-Rex
\item FlinkCEP
\end{itemize}

The following competitor systems remain to be investigated.
\begin{itemize}
\item Cayuga. Code in C++ available at \url{https://sourceforge.net/p/cayuga/code/HEAD/tree/}. Unclear whether it still compiles. SEQ queries should not be a problem. Unclear whether Kleene closure (under our semantics) can be expressed. Cayuga uses skip-till-any-match selection, and reuse as consumption policy.

  We will not compare against Cayuga (too old). Argument: only compare against sytems after 2010.
\item Streaming SQL: either Flink or Spark.
  \begin{itemize}
  \item From the discussion with Marco, it is not possible to encode SEQ queries in Spark structured streaming because stream-to-stream joins are only possible with equality predicates (by contrast SEQ requires inequality comparisons). Also, spark structured streaming does not support the MATCH RECOGNIZE clause through which CEP-like constructs can be expressed in SQL.
  \item Flink SQL does support MATCH RECOGNIZE, and would be another competitor. According to \url{https://ci.apache.org/projects/flink/flink-docs-master/docs/dev/table/sql/queries/match_recognize/#installation-guide}, MATCH RECOGNIZE is implemented internally using FLINK CEP. Moreover, not all of MATCH RECOGNIZE is supported. Since we compare directly against FLINK CEP, there is no point in comparing against Flink SQL. 

    
  \end{itemize}
\item SIDDHI  \url{https://github.com/siddhi-io/siddhi}.  Siddhi is a cloud native Streaming and Complex Event Processing engine that understands Streaming SQL queries in order to capture events from diverse data sources, process them, detect complex conditions, and publish output to various endpoints in real time. Ssupport for complex event detection is documented at the following sites
  \begin{itemize}
  \item \url{https://siddhi.io/en/v5.1/docs/query-guide/#pattern}
  \item \url{ https://siddhi.io/en/v5.1/docs/query-guide/#sequence}
  \end{itemize}
\item EIRES. Implementation for the SIGMOD 2021 paper \emph{Efficient Integration of Remote Data in Event Stream Processing}. In this paper, authors consider a SASE-like CEP lanaguage, to which they add the ability to consult external datasources that are not being updated. They study the problem of how latency can be minized using two classical technique: prefetching and lazy evaluation. They consider an automaton-based execution model (where states buffer events), where state transitions can fetch tuples from remote data sources. They propose a probabilistic cost model to choose between prefetching and lazy evaluation.
  
  Implemenation is availble at https://github.com/zbjob/EIRES. Written in C++. Does seem to have a query language and generic (automaton-based) execution model. Since the model is optimized for interaction with external data sources, the comparison may not be fair.
\end{itemize}

The following papers have been considered but either (i) do not have an implementation or (ii) have an implementation that is custom-tailored specifically for experiments (query + data) of the paper. In case (ii) the implementation hence cannot easily be retargeted to other query or data workloads.

I list here only the ``short'' paper names, see \url{https://github.com/DomagojVrgoc/CEP/blob/master/systems/summary.md} for full descriptions.

\begin{itemize}
\item ZStream
\item NextCEP
\item DistCED
\item The CEP papers originating from WPI (in SIGMOD 2016, 2017, 2019, 2021 and VLDB 2018)
\item Various papers on evaluating CEP in a parallel/distributed manner. (See the ``various papers''section at the above-mentioned URL).
\item Papers that try to forecast CEP patterns (based on learning)
\item SAP ESP. Described in the paper Multi-Query Optimization for Complex Event Processing in SAP ESP, ICDE 2017

Considers multi-query optimization for complex event patterns that allow SEQ, OR, AND, NEG. They express this as a cost-based query optimization problem.

Implementation: SAP ESP (SAP Event Stream Processor) seems to include basic CEP pattern matching functionality: through the MATCHING clause.

It appears, however, that, while SAP offers 30-day trial versions of its producs, SAP ESP itself is no longer downloadable from its website (perhaps it was packaged as a different part of a software?)
\end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main/main"
%%% End:


==> sections/experiment-notes.tex <==
\subsection{Experiments: notes}

\andres{Here's a list of what I've done so far:}

\begin{enumerate}
	\item Im using 2 types of queries with different streams. First a sequence query and then a kleene query, both with varying lenghts.
	\item All streams have random noise in between, and all events are selected uniformly.
	\item Some streams lack the last event of the sequence, to test how good the systems are at handling very few matches.
	\item Tested systems with a fixed size stream (1M) and measured the time it took (inconsistent IMO).
	\item Tested systems by putting a fixed timeout on the engine and giving it as many events as it could handle (much more consistent). For this test, I first loaded the entire stream onto memory.
	\item For Esper and SASE, I'm printing the first 10 matches (what is considered "first" varies by system).
	\item Flink uses different semantics for consumption, so against it I'm only outputting one Match.
	\item Same applies for the stock market queries.
\end{enumerate}

Here is a dump of the meeting between Andres, Cristian, and Stijn concerning the final paremeters of the experiments, and their conclusions.


\paragraph*{Experimental setup, to say:}
\begin{itemize}
\item  same query with same semantics, if possible. We will explicitly mention if semantics differs
\item
  stream is loaded in memory prior to processing, for all systems. We hence read from memory
\item
  We process as many events as we can in 60 seconds. Explain that the more we read, the worse competitors behave. Therefore, processing as much as possible in 60 seconds is better for competitors.
\item
  Explain how memory is measured
\item 
Throughput and memory consumption are measured separately
\item
  Measurements are 3 times, averages reported.
\end{itemize}

\paragraph*{SEQ WITH OUTPUTS}
\begin{itemize}
\item
  Keep the noise constant (and don’t report those). Only report for 6 noise events
\item
  Discussed parameters:
\begin{itemize}
\item
  \# of events: 3, 5, 7
\item
  \# of noise events: 6
\item
  window length: 100, 200, 300
\end{itemize}
\item
  Performance measures: throughput, but also enumeration time, preprocessing time, memory usage
\item
  Conclusions:
  \begin{itemize}
  \item
    As the number of events increases, CORE decreases linearly, other decrease exponentially
  \item
    Space is constant, but not in other case
  \item
    To comment: Enumeration time and preprocessing time is different. We are slower in enumerating. This is reasonable because we need to “decompress” the data structure, but they have the match.
  \end{itemize}
\end{itemize}

\paragraph*{SEQ NO MATCHES}
(needed because SASE/ESPER have default consumption policy so that they “start again” once a match is found).

Discussed parameters:
  \begin{itemize}
  \item
    \# of events: 3, 5, 7 (we will only report one, preferably 3 if this shows our conclusions)
  \item
    \# of noise events: 6
window length: 100, 200, 300
  \end{itemize}
Performance measures: throughput (but ignore memory usage, enumeration time)

Conclusions:
As the window length increases, CORE remains constant, other decrease exponentially

\paragraph*{SEL + ALL SEQ NO MATCHES}
Idea: selection strategy  = performance optimization. So here compare CORE (ALL) with the default sel strategy of Sase (Next) / Esper (MAX). Performance of competing systems improves, but is still beaten by CORE without selection strategy.

Discussed parameters:
  \begin{itemize}
  \item
    \# of events: 3, 5, 7 (we will only report one, preferably 3 if this shows our conclusions)
  \item
    \# of noise events: 6
  \item
    window length: 100, 200, 300
  \item
    Performance measures: throughput (but ignore memory usage, enumeration time)
  \end{itemize}

  
\paragraph*{KLEENE}
Discussed parameters:
  \begin{itemize}
  \item
    \# of events: 3, 5, 7 (if 7 can be run)
  \item
    \# of noise events: 6
  \item
    window length: 100 (fixed)
  \item
    Performance measures: throughput (but ignore memory usage, enumeration time)
  \end{itemize}

\paragraph*{DISJUNCTION}
Discussed parameters:
  \begin{itemize}
  \item
    \# of events: 4, 7, 10 
  \item
    \# of noise events: 6
  \item
    window length: 100 (fixed)
  \item
    Performance measures: throughput (but ignore memory usage, enumeration time)
  \end{itemize}

\paragraph*{STOCK}
with given parameters, but now with new way of calculating throughput



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main/main"
%%% End:



